Under the Hood of Transformer Networks for Trajectory Forecasting

Transformer Networks have established themselves as the de-facto state-of-the-art for trajectory forecasting but there is currently no systematic study on their capability to model the motion patterns of people, without interactions with other individuals nor the social context. This paper proposes the first in-depth study of Transformer Networks (TF) and Bidirectional Transformers (BERT) for the forecasting of the individual motion of people, without bells and whistles. We conduct an exhaustive evaluation of input/output representations, problem formulations and sequence modeling, including a novel analysis of their capability to predict multi-modal futures. Out of comparative evaluation on the ETH+UCY benchmark, both TF and BERT are top performers in predicting individual motions, definitely overcoming RNNs and LSTMs. Furthermore, they remain within a narrow margin wrt more complex techniques, which include both social interactions and scene contexts. Source code will be released for all conducted experiments.

==> sections/abstract.tex <==
%
%Forecasting the people motion is an important but complex task, which has been addressed so far with a variety of temporal and spatio-temporal models. 
%
\begin{abstract}

\FG{Write new abstract. The current one is from our ICPR.}
    
\FG{Main message for the abstract: By now Transformer Networks have established themselves as the \emph{de facto} state-of-the-art for trajectory forecasting but there it no study focusing on their capability to predict individuals, thus w/o social models and context. We consider transformer networks w/o bells and whistles, an exhaustive evaluation of frameworks and specifically focus on the capability of these models to address multi-modal futures.\\}
Most recent successes on forecasting the people motion are based on LSTM models and \emph{all} most recent progress has been achieved by modelling the social interaction among people and the people interaction with the scene.
%nearly saturating a reference dataset ETH+UCY.
%
We question the use of the LSTM models and propose the novel use of Transformer Networks for trajectory forecasting. This is a fundamental switch from the sequential step-by-step processing of LSTMs to the only-attention-based memory mechanisms of Transformers. In particular, we consider both the original Transformer Network (TF) and the larger Bidirectional Transformer (BERT), state-of-the-art on all natural language processing tasks.
%
Our proposed Transformers predict the trajectories of the individual people in the scene. These are ``simple'' models because each person is modelled separately without any complex human-human nor scene interaction terms. In particular, the TF model \emph{without bells and whistles} yields the best score on the largest and most challenging trajectory forecasting benchmark of TrajNet~\cite{sadeghiankosaraju2018trajnet}. Additionally, its extension which predicts multiple plausible future trajectories performs on par with more engineered techniques on the 5 datasets of ETH~\cite{pellegrini2009iccv}+UCY~\cite{lerner2007crowds}. Finally, we show that Transformers may deal with missing observations, as it may be the case with real sensor data.
Code is available at \texttt{github.com/FGiuliari/Trajectory-Transformer}.

\FG{Add (this is the agreed of new contributions of this work):\\
- analyze LSTM and TF w/ Regressive, Gaussian, Quantized\\
- analyze BERT Autoregressive VS One Shot prediction\\
- analyze TF and BERT with Speed or Relative Positions\\
- study multi-modality, introduce trans-rotated zara2\\
- Distribution of train and test end points\\
- Distr of BERT-os with train obs (end points)\\
- Distr of BERT-os with test obs (end points)\\
- Bert with grid end points\\
}

\end{abstract}


\iffalse
Forecasting the people motion is an important but complex task, which has been addressed so far with a variety of temporal and spatio-temporal models. Most recent successes are based on LSTM models and \emph{all} most recent progress has been achieved by modelling the social interaction among people and the people interaction with the scene.
%nearly saturating a reference dataset ETH+UCY.
%
We question the use of the LSTM models and propose the novel use of Transformer Networks for trajectory forecasting. This is a fundamental switch from the sequential step-by-step processing of LSTMs to the only-attention-based memory mechanisms of Transformers. In particular, we consider both the original Transformer Network (TF) and the larger Bidirectional Transformer (BERT), state-of-the-art on all natural language processing tasks.
%
Our proposed Transformers predict the trajectories of the individual people in the scene. These are ``simple'' model because each person is modelled separately without any complex human-human nor scene interaction terms. In particular, the TF model \emph{without bells and whistles} yields the best score on the largest and most challenging trajectory forecasting benchmark of TrajNet~\cite{sadeghiankosaraju2018trajnet}. Additionally, its extension which predicts multiple plausible future trajectories performs on par with more engineered techniques on the 5 datasets of ETH~\cite{pellegrini2009iccv}+UCY~\cite{lerner2007crowds}. Finally, we show that Transformers may deal with missing observations, as it may be the case with real sensor data.
\fi
%These results call for the importance of temporal modelling for progress in the field.

%Leveraging the recent progress of sequence modelling from NLP contexts, we model memory with attention and demonstrate that this better captures the non-linearities of long people trajectories. Our model 





==> sections/extra.tex <==
\LeoP{
\subsubsection{Experiments with BERT one shot \label{Sec:multimodal}}
We here conduct an analysis on ETH/UCY and, mainly using BERT one shot, we try to show some interesting insights on the way trajectories are predicted. The plots that you can see in Fig.~\ref{fig:Mult1} -~\ref{fig:Mult2} -~\ref{fig:RandomB} have all a central element belonging to Zara2, which we used as test set in our analysis and that, as you may notice was transformed by us (with all ETH/UCY) to perform a better analysis. The motivation because we decided to modify the dataset is that we wanted to have an easy way of finding similar trajectories without accounting every time that the two elements may be extremely far or rotated in space. For this reason our new ETH/UCY is such that every trajectory starts in the origin of the plane (0, 0) and is rotated with angle such that the 8th step (which in ETH/UCY is generally taken as last element of the input when running a model) is always on the positive x-axes, thus of coordinates $el_{8th} = (+pos\_num, 0)$.
After doing this we decided that the metric to adopt to estimate the similarity between trajectories would be the L2 norm, therefore if the L2 norm between two trajectories is low we could assume they are relatively similar. Now we here notice that this modified-ETH/UCY is interesting to use for an analysis and, training on it the models presented in this paper, we didn't find any significant degradation in the performance metrics. 
The note to make is that would not be rewarding to use this dataset for real time predictions since there would be necessary to rotate and translate back every output, but all this is out of our purpose. Starting from Fig.~\ref{fig:Mult1} you can see that in the first row we show trajectories that we call 'similar' or 'multimodal' from the training dataset. Indeed, selecting a central element from test that we cal $el25$, computing the L2 norm between the first 8 steps of $el$ (its green part) and every element in the train dataset we first understand which train elements are most similar to the past of $el$ (which is what we feed any model) and call this procedure 'past analysis'. After that we repeat this measuration between the steps 9-20th of $el$ (which are in black and are generally what we want to predict with the models) and again we undestand which elements in train hold a similar future to $el$ and we call this procedure 'future analysis'. Done that, we have ranked train trajectories for the past and the future dinstance from $el$ and, selected an index n which here shown is 200, we assign the label 'similar' to the trajectories in train that were in the top\_n in the past and in the future analysis. When instead trajectories were in the top\_n in the past analysis but not in the future analysis, we call these trajectories "multimodal" since they differ significantly from $el$ but have the same past (so feed the past a model we would like it to grasp also these alternatives if trained on them). 
So in Fig.~\ref{fig:Mult1} a) and b) you clearly notice the more variety in b) and the fact that we have different direction but with very similar past (the blue part).
Below, in c) and d) you can see how our BERT one shot reconstructs the "similar" and "multimodal" tracks given their true endpoints (and the past of $el$). We believe the result is of a good quality but we must notice that the irregularities in the original tracks, that for example have a decise change in direction just in the last few steps, is not captures from the model. Indeed the regularity of this predicted plots clearly shows that the predicted trakcs are smooth and you will notice extremely rarealy present the typical final irregular change of direction.
In e), f), g) and h), analyzing the endpoints distributions in the first two, and then the entire distributions, you may see that the multimodal elements are clearly more diverse and that, since the training procedure did observe these elements, we expect it would reflect in the predicted distribution of endpoints at least.
We now go to Fig.~\ref{fig:Mult2}, where in a) we can see how BERT one shot is able to reconstruct paths from endpoints of neighbours test elements. With b) that shows generated trajectories from estimated endpoints, we may vary that the standard generation from BERT one shot hold a pretty high diversity. In fact in c) and d) we see that the estimated elements endpoints is much wider than that of 'similar'/neighbour test tracks. In e) and f) you can again see the difference in the 'similar' tracks distribution and the distribution that BERT one shot is able to give of the endpoints. This means that, at a certain degree, this model capture enough multimodality to give a good variation of endpoints.
Finally, again trying to understand the quality of our BERT one shot, we did generate endpoints with a normal distribution and watching Fig.~\ref{fig:RandomB} you can see how the model recontructs trajectories all around, adjusting the speed based on the endpoints and finally presenting the typical irregularities at the end of our tracks.}

\begin{figure*}[t]
    \centering
   \includegraphics[width= \linewidth]{./Figures/25train.png}
    \caption{The element in green and black is from Zara2}
    \label{fig:Mult1}
\end{figure*}{}
\begin{figure*}[t]
    \centering
    \includegraphics[width= 0.5 \linewidth]{./Figures/25paths.png}
    \caption{The element in green and black is from Zara2}
    \label{fig:Mult2}
\end{figure*}{}

%Take out GT from this figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.5 \linewidth]{./Figures/RandomBertOnes.png}
    \caption{Reconstruction of trjactories given random endpoints for an element in Zara2}
    \label{fig:RandomB}
\end{figure*}{}



\begin{figure*}[t]
    \centering
   \includegraphics[width= \linewidth]{./Figures/Leo_images/clus_1.png}
    \caption{}
    \label{fig:cl1}
\end{figure*}{}
\begin{figure*}[t]
    \centering
    \includegraphics[width=  \linewidth]{./Figures/Leo_images/clus_2.png}
    \caption{}
    \label{fig:cl2}
\end{figure*}{}

%Take out GT from this figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{./Figures/Leo_images/clus_3.png}
    \caption{}
    \label{fig:cl3}
\end{figure*}{}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{./Figures/Leo_images/clus_4.png}
    \caption{}
    \label{fig:cl4}
\end{figure*}{}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{./Figures/Leo_images/clus_5.png}
    \caption{}
    \label{fig:cl5}
\end{figure*}{}

\subsubsection*{Clustering on the distributions}\\

\FG{Please structure this section: (1) first an intro: what we want to show, why we pick bert-os(need to point to its performance in previous tables); (2) then a paragraph on the new constructed dataset: first the objective and then how we constructed the dataset (this roughly includes points 1 and 2 of Leonardo but need to select a simpler story from the current text); (3) then the actual analysis. Please write in paragraphs (more paragraphs for the analysis after the initial 2), not in bullets.}
Starting from an original past trajectory of 8 steps, we now observe how BERT one shot is able to reconstruct the futures both in the train dataset and the test dataset. \newline
\begin{itemize}
    \item 1) \textit{The selected central trajectories}. As you may see in figures ~\ref{fig:cl1} -~\ref{fig:cl2} the plots present always a central trajectory. These 5 total centroids have been selected through a clustering process to ensure we capture 5 different trajectories in Zara2\_Modified. \FG{No need to put so much emphasis on clustering. The clustering was a simple tool. Most important is the data preparation and especially the motivation, which should be introduced first in this section.}
    \item 2) \textit{The clustering process}. We analyzed the train set and we observed for every trajectory the first 8 points. From here we collapsed every point in a 2D representation as $point = (x_8, Var(\alpha))$ where $Var(\alpha)$ is the variance of the vector of the angles $\alpha_i$ between each different step from the 1st to the 8th $(Var( [ \alpha_{0-1}, ...,\alpha_{7-8}])$. \FG{Most likely, at this point in the paper we don't want to define new formalism. Just describe the procedure in words, spelling out what you want to achieve and how you proceed to achieve it.} The reason is that in this way we are considering as an important characteristic of a trajectory the 8th step (that we always know is a positive number from how we constructed the Zara2\_Modified) as a speed marker, and, with the variance, in a sense the general curvature in the first 8 steps. From here we performed K-Means on the points and, after observing an Elbow between 4 and 6, we extracted 6 centroids also expecting to have captured some noisy trajectory. From here we did perform the same transformation in 2D for Zara2\_Modified, but now we selected the 6 nearest points to our 6 centroids in train. This was to try to extract different test trajectories having looked at the train general structure that was fed to the model. These 6 centroids were finally converted in the original trajectories and you can see 5 of them in the images, the 6th was, as Fig. ~\ref{fig:cl1} [2] a noisy element of our dataset, so we decided to not include it in our analysis.
    \item  3) \textit{The multimodal trajectories}. The a) sections in the figures ~\ref{fig:cl1}-~\ref{fig:cl2} show each a centroid trajectory sourrounded by a set of blue and red tracks. \FG{Please express the concept you want to achieve first; then how you proceed to achieve it. This is named "top-down" and is really important for the reader understanding.} Every track showed, except for the centroid, is from the training data and every item has been divided in past 8 steps, blue part, and future 12 steps, red part. The representation is called 'multimodal trajectories for an elemen' because these trajectories are selected in the following way. Considering that our dataset, train and test, have been translated and rotated, we decided we could use the L2 norm between tracks to identify now more easily similar tracks. Indeed now similar trajectories will be all in the same region of space and not far away. We then computed the L2 distance between the centroids of Zara2\_Modified and we found which ones are the nearest 200 for distance in the past (so L2 distance between the first 8 steps) and for the future (L2 distance between the futures 12 steps). From this we decided to define as 'multimodal' those tracks that were in top 200 in the past (that means they had very similar start and so input for our models), but that variate more in the futures such that they do not reappear in the top 200. You can then see, among the different figures, that we captures very different distibutions from our centroid and we note that, for Fig~\ref{fig:cl2} they are incredibly different that the very short trajectory we have. 
    \item  4) \textit{BERT one shot reconstruction from the enpoints}. \FG{Adopt a top-down structure for this paragraph.} The b) sections in the figures~\ref{fig:cl1}-~\ref{fig:cl2} show each again the centroid, but this time sorrounded by red recontruction from BERT one shot. This reconstruction has been performed using BERT one shot based on the endpoints from a) section and the method of relative positions (not velocities that we saw obtains worse results). From here, before commenting we have to notice that the model is such that it will predict again an 'adjusted' endpoint, so for example in Fig~\ref{fig:cl1} [2] that we mention has a noisy input, the endpoints are modified such that the reconstruction is worse that the other cases. In the other figures we notice that the reconstruction is mainly composed of smooth lines and the trakcs are always plausible solutions to reach the endpoints. We have not completely ireegular tracks, and even the ones in in Fig~\ref{fig:cl2} where you can notice irregular endings, are indeed normal since we noticed many similar trends in the training data. We remember that this section b) comprises endpoints from the train data.
    \item  5) \textit{The neighbours test data}. In the sections c) we presented the local distribution in the test data regarding the sorrounding points to the centroid. The procedure to find the neighbour points is the same as for the multimodal and we show here how mostly regular is the test data we are feeding. From here we want to understand if the model is able to capture a more complex distribution than what we expect from the test data.
    \item  6) \textit{BERT one shot samples resutls in Zara\_Modified}. Indeed in figure d) we can notice that using BERT one shot and approximating the endpoints, sampling many of them, we then arrive to a resulting distribution of endpoints much wider than the original section), indicating that the model was able, thorugh training, to capture a wide variety of trajectories.
\end{itemize}




==> sections/proposed_approach.tex <==



\section{The Transformer Model}\label{sec:method}

\begin{figure*}[!t]
\centering
  \includegraphics[width=0.40\textwidth, height = 4.5cm]{Figures/LSTM__fix.png}
  \includegraphics[width=0.59 \textwidth, height = 4.5cm]{Figures/TF__.png}
\vspace{-0.5cm}
\caption{Model illustration of LSTM~(\textit{left}) and TF~(\textit{right}). At each time step, LSTM leverages the current-frame information and its hidden state. By contrast, TF leverages the encoder representation of the observed input positions and the previously predicted outputs. In purple and grey are the self-attention and encoder-decoder attention modules, that allow TF to learn on which past position it needs to focus to predict a correct trajectory.
}
\label{fig:lstm_tf}
%Upon an observation time, when the TF and BERT model of each person ``sees'' the motion history of itsself, they start predicting the future. At each prediction time-step, each person TF and BERT process their own predicted position auto-regressively.
\vspace{-0.2cm}
\end{figure*}




%  \begin{figure*}[t]
% 	\begin{center}
% 	    \includegraphics[width=1\linewidth]{Figures/Model_picture.pdf}
% 	   % \decoRule
% 	\end{center}
% % 	\vspace{-5pt}
% 	\caption{.}\label{fig:prop-appro}
%  	%\vspace{-16pt}
% \end{figure*}




% \begin{figure}[!htb]
% \minipage{0.32\textwidth}
%   \includegraphics[width=\linewidth]{Figures/LSTM.pdf}
%   \caption{}\label{fig:awesome_image1}
% \endminipage\hfill
% \minipage{0.32\textwidth}
%   \includegraphics[width=\linewidth]{Figures/BERT.pdf}
%   \caption{}\label{fig:awesome_image2}
% \endminipage\hfill
% \minipage{0.5\textwidth}%
%   \includegraphics[width=\linewidth]{Figures/tf.pdf}
%   \caption{}\label{fig:awesome_image3}
% \endminipage
% \end{figure}



% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.33\textwidth]{Figures/LSTM.pdf}} 
%     \subfigure[]{\includegraphics[width=0.33\textwidth]{Figures/LSTM.pdf}} 
%     \subfigure[]{\includegraphics[width=0.33\textwidth]{Figures/LSTM.pdf}}
%     \caption{(a) blah (b) blah (c) blah (d) blah}
%     \label{fig:foobar}
% \end{figure}



We propose a multi-agent framework where each person is modelled by an instance of our transformer network. Each Transformer Network predicts the future motion of the person as a result of its previous motion.

We describe in this section the model input and output (Sec.~\ref{sec:inout}), the encoder-decoder Transformer Network (TF) (Sec.~\ref{sec:encdec}) and the just-encoder BERT model (Sec.~\ref{sec:bert}) and the implementation details (Sec.~\ref{sec:modtrain}). %Please refer to Fig.~\ref{fig:lstm_tf} for an overall illustration of our model.

\subsection{AB}\label{sec:in1}
\subsection{BC}\label{sec:in2}
\subsection{CD}\label{sec:in3}

\subsection{Model input and output}\label{sec:inoutAA}

For each person, the transformer network outputs the predicted future positions by processing their current and prior positions (observations or motion history). We detail here each of the input and output information and parallel those with the established LSTM, with reference to Fig.~\ref{fig:lstm_tf}.

% Note: both the TF and BERT models only consider the motion histories of each person separately, without awareness of the social person-person interaction~\cite{some-cites}, nor awareness of the context~\cite{sr-lstm,trajectronpp}.


\paragraph{Observed and predicted trajectories}
In formal terms, for person $i$, we are provided a set $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^0_{t=-(T_{obs}-1)}$ of $T_{obs}$ observed current and prior positions in Cartesian coordinates $\mathbf{x}\in\mathcal{R}^2$, and we are required to predict a set $\mathcal{T}_{pred}=\{\mathbf{x}^{(i)}_t\}^{T_{pred}}_{t=1}$ of $T_{pred}$ predicted positions. %$W_{\mathbf{x}}$
In order to let the transformer deal with the input, this is embedded onto a higher $D$-dimensional space by means of a linear projection %function $\phi$ 
with a matrix of weights $W_{\mathbf{x}}$, i.e., $\mathbf{e}_{obs}^{(i,t)} =  \mathbf{x}^{(i)^{\intercal}}_t  W_{\mathbf{x}}$.

%, followed by a ReLU activation function:
%\begin{equation}
%    \mathbf{e}_{obs}^{(i,t)} = \phi \left( %\mathbf{x}^{(i)}_t,W_{\mathbf{x}} \right)
%\end{equation}
In the same way, the output of our transformer model for person $i$ at time $t$ is the $D$-dimensional vector $\mathbf{e}_{pred}^{(i,t)}$, which is back-projected to the Cartesian person coordinates $\mathbf{x}^{(i)}_t$. LSTM and TF share this aspect.






% In formal terms, for person $i$, we are provided a set $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^0_{t=-(T_{obs}-1)}$ of $T_{obs}$ observed current and prior positions in Cartesian coordinates $\mathbf{x}\in\mathcal{R}^2$, and we are required to predict a set $\mathcal{T}_{pred}=\{\mathbf{x}^{(i)}_t\}^{T_{pred}}_{t=1}$ of $T_{pred}$ predicted positions. 
% \mc{In order to let the transformer deal with the input, this is embedded onto a higher $D$-dimensional space by means of a linear projection %function $\phi$ 
% with a matrix of weights $W_{\mathbf{x}}$, i.e., $\mathbf{e}_{obs}^{(i,t)} =  \mathbf{x}^{(i)}_t^{\intercal}W_{\mathbf{x}}$.}
% %, followed by a ReLU activation function:
% %\begin{equation}
% %    \mathbf{e}_{obs}^{(i,t)} = \phi \left( %\mathbf{x}^{(i)}_t,W_{\mathbf{x}} \right)
% %\end{equation}
% In the same way, the output of our transformer model for person $i$ at time $t$ is the $D$-dimensional vector $\mathbf{e}_{pred}^{(i,t)}$, which is back-projected to the Cartesian person coordinates $\mathbf{x}^{(i)}_t$. LSTM and TF share this aspect.


% In formal terms, for person $i$, we are provided a set $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^0_{t=-(T_{obs}-1)}$ of $T_{obs}$ observed current and prior positions in Cartesian coordinates $\mathbf{x}\in\mathcal{R}^2$, and we are required to predict a set $\mathcal{T}_{pred}=\{\mathbf{x}^{(i)}_t\}^{T_{pred}}_{t=1}$ of $T_{pred}$ predicted positions.
% \mc{In order to let the transformer deal with the input, this is embedded onto a higher $D$-dimensional space by means of a linear projection function $\phi$ with a matrix of weights $W_{\mathbf{x}}$, followed by a ReLU activation function:
% \begin{equation}
%     \mathbf{e}_{obs}^{(i,t)} = \phi \left( \mathbf{x}^{(i)}_t,W_{\mathbf{x}} \right)
% \end{equation}}
% In the same way, the output of our transformer model for person $i$ at time $t$ is the $D$-dimensional vector $\mathbf{e}_{pred}^{(i,t)}$, which is back-projected to the Cartesian person coordinates $\mathbf{x}^{(i)}_t$. LSTM and TF share this aspect



\paragraph{Positional encoding}
The transformer encodes time for each past and future time instant $t$ with a ``positional encoding''. In other words, each input embedding $\mathbf{e}_{obs}^{(i,t)}$ is time-stamped with its time $t$. The same encoding is used to prompt the model to predict into future instants, as we detail in the next section.

More formally, the input embedding $\mathbf{e}_{obs}^{(i,t)}$ is time-stamped at time $t$ by adding a positional encoding vector $\mathbf{p}^{t}$, of the same dimensionality $D$:
%\begin{equation}\label{eq:posenc}
$
    \mathbf{\xi}_{obs}^{(i,t)} = \mathbf{p}^{t} + \mathbf{e}_{obs}^{(i,t)}
$
%\end{equation}

We use sine/cosine functions to define $\mathbf{p}^{t}$ as in~\cite{TransformersNIPS17}:
%We follow the formulation of \cite{TransformersNIPS17} and use sine/cosine functions to define $\mathbf{p}^{t}$:
\begin{align}
    &\mathbf{p}^{t}=\left\{ p_{t,d} \right\}_{d=1}^{D}\\
    &\text{where}\quad
    %
        p_{t,d}=\left\{
        \begin{tabular}{lr}
        sin$\left(\frac{t}{10000^{d/D}}\right)$ & for $d$ even \\
        cos$\left(\frac{t}{10000^{d/D}}\right)$ & for $d$ odd
        \end{tabular}
    \right.
    %
\end{align}
In other words, each dimension of the positional encoding varies in time according to a sinusoid of different frequency, from $2\pi$ to $10000 \cdot 2\pi$. This ensures a unique time stamp for sequences of up to 10000 elements and extends unseen lengths of sequences. %and allow the model to process input by relative positions, i.e.\ for a given offset $t_o$ the encoding vector $\mathbf{p}^{t+t_o}$ may be represented as a linear function of $\mathbf{p}^{t}$.

In this aspect, TF differs greatly from LSTM, cf.\ Fig.~\ref{fig:lstm_tf}. LSTM processes the input sequentially and the order of input positions determine the flow of time. It does not therefore need a positional encoding. However, LSTM needs to ``unroll'' at training time, i.e.\ back-propagate the signal sequentially across the LSTM blocks processing the observations. By contrast, the training of TF is parallelizable.
%TF may learn from all time instants in parallel, which results in more efficient and scalable training.

Notably, thanks to the positional encoding which time-stamps the input, TF may deal with missing observations.  Missing data is just neglected, but the model is aware of the relative time-stamps of the presented observations. In Sec.~\ref{Sec:exp}, we experiment on this unique feature, important when dealing with real sensor data.



\paragraph{Full comparison: Models VS Frameworks}

To have a complete analysis, we evaluated different architectures: LSTM, Transformer and BERT, with a deterministic or probabilistic framework. 
In the first approach (Regressive) the models do directly position or speed regression while in the second case, a probability distribution is learned from which to sample the next prediction.

The latter framework is divided into two approaches: the Gaussian, often implemented in the literature, where the parameters of a bi-dimensional Gaussian are predicted, and the Quantized approach where the inputs are quantized into classes and the input data represented as one-hot-vectors.

%(Before it was written)
%We test both approaches and  confirm  the  better  performance  of  regression.  However, a  classification  approach,  which  we  dub  TFq,  provides  a probabilistic output across the quantized motions. We leverage TFq to sample multiple future  predictions, which we   assess both quantitatively and qualitatively. The predictions of TFq are multi-modal, as we illustrate in Sec. VI.

%(Actually i would change for)
We test both approaches and the results are consistent for most of the methods. However, we leverage probabilistic methods to sample multiple future predictions, which we assess both quantitatively and qualitative. The predictions of them are multi-modal, as we illustrate in Sec.~\ref{Sec:exp}.


BERT's architecture allows us to implement two different versions. The first one, similar to Transformer, predicts in a \textit{autoregressive} way the single future position, while the second one predicts all the $\mathcal{T}_{pred}$ future outputs \textit{jointly}. 
With the first approach the model learns a marginal distribution for the specific time instant to be predicted, conditioned by past outputs, while in the second approach it learns a joint distribution for each time instant, which also learns the mutual dependencies among the time dimensions.


%TF$_q$ outputs softmax'ed probabilities which differ from the Gaussian LSTM~\cite{alahi2016cvpr} probabilistic output. The TF$_q$ outputs are in fact multi-modal, as being generated directly by a deep neural network, while Gaussian LSTM only predicts means and variances of Gaussians, forcing the predictions to a single mode. We illustrate this in Sec.~\ref{Sec:exp}.



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{./Figures/EncDecModel.JPEG}
% \caption{Upon an observation time, when the TF and BERT model of each person ``sees'' the motion history of itsself, they start predicting the future. At each prediction time-step, each person TF and BERT process their own predicted position auto-regressively. \todo{Irtiza: please update this figure.}}
% \label{fig:encdecmodel}
% \end{figure}




\subsection{Encoder-decoder Transformer (TF)}\label{sec:encdec}

As illustrated in Fig.~\ref{fig:lstm_tf}, TF is a modular architecture, where both the encoder and the decoder are composed of 6 layers, each containing three building blocks: \textbf{i.}\ an attention module, \textbf{ii.}\ a feed-forward fully-connected module, and \textbf{iii.}\ two residual connections after each of the previous blocks.

The capability of the network to capture sequence non-linearities lies mainly in the attention modules. Within each attention module, an entry of a sequence, named ``query'' (Q), is compared to all other sequence entries, named ``keys'' (K) by a scaled dot product, scaled by the equal query and key $d_k$ embedding dimensionality. The output is then used to weight the same sequence entries, named now ``values'' (V). Attention is therefore given by the equation:
%In practice, each sequence entry is considered as query, and all entries are gathered into matrices of queries \emph{Q}, keys \emph{K} and values \emph{V}, to yield attention according to equation:
%\vspace{-0.3cm}
\begin{equation}\label{eq:att}
    \text{Attention}(Q,K,V)=softmax\left(\frac{Q K^T}{\sqrt{d_k}}\right)
\end{equation}

The goal of the encoding stage is to create a representation for the observation sequence, which makes the model \emph{memory}. To this goal, after the encoding of the $T_{obs}$ input embeddings $\mathbf{\xi}_{s}^{(i,t)}$, the network outputs two vectors of keys $K_{enc}$ and values $V_{enc}$ which would be passed on to the decoder stage.

The decoder predicts auto-regressively the future track positions. At each new prediction step, a new decoder query $Q_{dec}$ is compared against the encoder keys $K_{enc}$ and values $V_{enc}$ according to Eq.~\eqref{eq:att} (encoder-decoder attention) and against the previous decoder prediction (self-attention).
%, to yield the next-step prediction.

Note the important difference w.r.t.\ LSTM: TF maintains the encoding output (memory) separate from the decoded sequence, while LSTM accumulates both into its hidden state, steering what to memorize or forget at each time. We believe this may contribute to explain how TF outperforms LSTM in long-term horizon predictions, cf.\ Sec.~\ref{Sec:exp}.



% \begin{figure}[!ht]
% \centering
%   \includegraphics[width=0.43 \linewidth, height = 4.5cm]{Figures/BERT_.png}
% \vspace{-0.3cm}
% \caption{Model illustration of BERT}\label{fig:bert}
% \end{figure}



\subsection{BERT}\label{sec:bert}

We consider for trajectory forecasting a second Transformer model, BERT~\cite{BERT19}.
Differently from TF, BERT is only composed of an encoder and it trains and infers thanks to a masking mechanism. In other words, the model hides (masks) from the self-attention the output positions which it targets for prediction as the TF decoder also does.
During training the model learns to predict masked positions. At inference, the model output predictions for the masked outputs.

BERT is the \textit{de-facto} reference model for state-of-the-art NLP methods, but larger than TF ($\sim$2.2 times larger). As we would illustrate in Sec.~\ref{Sec:exp}, training BERT on the current largest trajectory forecasting benchmarks does not keep up to the expectations. We draw inspiration from transfer learning and test therefore also how a BERT pre-trained on an NLP task performs on the target task. In particular, we take the lower-cased English text using Whole-Word-Masking; we substitute for the word embedding from dictionary keys with similar linear modules encoding ($x$,$y$) positions; and then we similarly convert also the output into ($x$,$y$) positions.

% At inference time, we apply the same approach, passing as input the observed values and mask tokens for the positions to predict.



\subsection{Implementation details}\label{sec:modtrain}

Our TF implementations adopts the parameters of the original Transformer Networks~\cite{TransformersNIPS17}, namely $d_{model}=512$, 6 layers and 8 attention heads. We adopt an L2-loss between the predicted and annotated pedestrian positions and train the network via backpropagation with the Adam optimizer, linear warm-up phase for the first 5 epoch and a decaying learning rate afterward; dropout value of 0.1.
The normalization of the network input influences its performance, as also maintained in \cite{zhang2019sr,graves2013generating}. So we normalize the people speeds by subtracting the mean and dividing by the standard deviation of the train set.
For the TF$_q$, we quantize the people motion by clustering speeds into 1000 joint ($x$,$y$) bins, then encode the position by 1000-way one-hot vectors. In order to get a good cluster granularity, we augment the training data by random scaling uniformly with scale $s\in[0.5,2]$.
%The lower-cased English text pre-trained BERT from which we fine-tune was trained extensively on the Wikipedia + BookCorpus for $\sim$1M steps

%In our work, we augment the training set by random rotations and scaling at training time. We model the random rotation by stochastic process and estimate the normalizing parameters by integrating away the rotation angle.

%Further to the performance, an added value of Trasformer networks is that training parallelizes across future prediction steps since the model does not need unrolling, as it is instead the case for LSTMs. 
%In practise, our networks trains in X hours for a time horizon of 12 future steps, while a corresponding LSTM takes X hours. However our model takes X hours when training to predict a 24 future step horizon, while LSTM turns instead to need X hours. Since in prediciting future, the long-term horizon is most important, this feature seems key in the choice of Transformers for pedestrian forecasting. 
%\todo{Irtiza:please complete the X's or comment this note.(from Francesco, i don't have the run times or the code for the LSTM. For Transformer the training time are about 30 min on my side and assuming one has enough vram the training is not affected by the forecasting horizon since all the forecasting are parallelized during training)}

%\todo{add: 1000 clusters by the use of k-means, then encode each person motion with a one-hot vector.}

%\todo{Francesco comment on BERT too, where the code is taken from and what parameters are then changed (and why)}

%\todo{add: We re-implement TF according to \cite{TransformersNIPS17}.}


